Distributed Learning Algorithms for Opportunistic Spectrum Access in Infrastructure-less Networks

An opportunistic spectrum access (OSA) for the infrastructure-less (or cognitive ad-hoc) network has received significant attention thanks to emerging paradigms such as the Internet of Things (IoTs) and smart grids. Research in this area has evolved from the \r{ho}rand algorithm requiring prior knowledge of the number of active secondary users (SUs) to the musical chair (MC) algorithm where the number of SUs are unknown and estimated independently at each SU. These works ignore the number of collisions in the network leading to wastage of power and bring down the effective life of battery operated SUs. In this paper, we develop algorithms for OSA that learn faster and incurs fewer number of collisions i.e. energy efficient. We consider two types of infrastructure-less decentralized networks: 1) static network where the number of SUs are fixed but unknown, and 2) dynamic network where SUs can independently enter or leave the network. We set up the problem as a multi-player mult-armed bandit and develop two distributed algorithms. The analysis shows that when all the SUs independently implement the proposed algorithms, the loss in throughput compared to the optimal throughput, i.e. regret, is a constant with high probability and significantly outperforms existing algorithms both in terms of regret and number of collisions. Fewer collisions make them ideally suitable for battery operated SU terminals. We validate our claims through exhaustive simulated experiments as well as through a realistic USRP based experiments in a real radio environment.

==> Discussion.tex <==
%In this section, we compare the proposed algorithms with existing algorithms with respect to network parameters.
%\begin{itemize}
%	\item synchronization between Tx and Rx
%	\item Tcc vs To
%	\item long sensing
%	\item constraints on user movement
%	\item sensing errors
%	\item No MAB
%	\item No of users are more than K
%	\item Changing channel statistics
%	\item Different reward for each user
%\end{itemize}


In this section, we compare the proposed algorithms and state-of-the-art MC \cite{MC} algorithm with respect to practical network constraints.

\begin{itemize}[leftmargin=*]
	
%	\item \textbf{Long Sensing:} The TSN and TDN algorithms as well as MC algorithm need sensing block such as energy detector to check the presence of primary users. In MC as well as TSN and TDN algorithms, the sensor block is also used to detect the SU collision. In the TSN algorithm, sensing block is effectively used to do long sensing for detecting whether the channel has been locked by SUs whereas in the TDN algorithm, it is used by the SUs entering the system to look for presence of a SU on any channel as well as to check whether the channel has been locked by other SUs. The long sensing concept is not new and has been discussed in few works such as \cite{quek}. We believe long sensing is an effective and practical way to efficiently utilize sensing hardware resources. The TSN and TDN algorithms employ long sensing to fasten orthogonalization of SUs in top channels without increasing the number of SU collisions as evident from the simulation and experimental results shown in previous sections.
		\item \textbf{U$>$N:} The trekking approach allows handling the case $U \ge N$, i.e., more number of SUs than channels. Indeed, if SU does not experience a collision-free transmission on the vacant band within the RH sub-phase of the CC phase, it is with high probability due to more SUs than the channels and the SU can leave and re-enter after a certain interval. In the MC or DMC algorithm, SUs will know this only after completing the learning phase which is significantly longer than RH sub-phase of the proposed algorithm, and it is unclear which SU will leave. Another major issue in the MC algorithm is that it will fail if SUs leave during the learning phase. This is because the MC algorithm uses collision count to estimate $U$. If SUs leave, collision count will not give a correct estimate of $U$. In the trekking approach, SUs need not know $U$ and works even if $U$ changes. 

	
	
	\item \textbf{Constraints on SU Entry/Exit:} The SUs cannot enter or exit the network during the learning phase of the MC algorithm. Else, the $U$ estimation may not correct leading to linear regret. Also, newly entered SUs need to wait for at most the duration of learning phase before beginning their data transmission. Such waiting time is significantly large since SUs are unlicensed users and remains active only for a short period. In the TDN algorithm, we do not impose such restriction on the entry and exit of the SUs making it feasible for a truly dynamic network.


	
	\item \textbf{Rendezvous:} The term rendezvous refers to the process of SU transmitter and receiver tuning themselves to communicate on an identical channel. The rendezvous allows SU receiver to tune it to the single channel instead of multiple channels simultaneously thereby making it less complex and compact. However, rendezvous is challenging in case of infrastructure-less networks due to lack of dedicated control channel between the transmitter and receiver \cite{MC,MEGA,prand,sdsp,seus,zhandi,
		tdfs,gai1,gai2,zandi,sumit1,eryk,bprand2}. The algorithm such as \cite{quek} makes it easy for SUs to achieve rendezvous due to deterministic sequential hopping based channel selection approach. However, it performs poorly as evident from simulation results. Compared to existing algorithms, the TSN and TDN algorithms offer easier rendezvous due to sequential hopping and trekking approach. It can be proved that the TSN and TDN  algorithms need $N$ time slots to establish rendezvous at the start of sequential hopping as well as once SUs lock itself on one of the top channels. For MC algorithm, rendezvous is not possible at all during the learning stage while it also needs $N$ time slots once SU locks itself on one of the top channels in MC stage. In case of remaining algorithms such as  \cite{MEGA,prand,sdsp,seus,zhandi,
		tdfs,gai1,gai2,zandi,sumit1,eryk,bprand2}, rendezvous is difficult due to the exploration-exploitation-collision trade-off based channel selection via multi-armed bandit algorithms. This makes the TSN and TDN algorithms a preferred choice when rendezvous is a critical factor for algorithm selection.
	
	\item \textbf{Orthogonalization Time and Regret:} The orthogonalization time refers to the number of time slots required for orthogonalization of SUs in the top channels. In the simulation and experimental results, we keep the orthogonalization time for the TSN, TDN and MC algorithms fixed and equal to 2000 time slots. However, orthogonalization time required for the MC algorithm is significantly longer than that of the TSN and TDN algorithms. This is because one of the aims of the learning stage of MC algorithm is to characterize channels and estimate $U$ and the time required for the same is $T_o$ \cite{MC}. In case of the TSN and TDN algorithms, estimation of $U$ is not needed, and the channel characterization is done during the collision-free sequential hopping phase of duration $T_{SH}$ slots. By comparing the $T_o$ expression in \cite{MC} with $T_{SH}$, we can easily show that $T_o > 2\cdot T_{SH}$. Since $T_{o}$ and $T_{SH}$ are the dominating terms in the regret expressions of the MC and TSN algorithms, respectively, we can show that the regret of the MC algorithm is at least two times the regret of TSN algorithm and the difference increases further in case of the dynamic networks. %The analytical comparison of the regret between the proposed and existing algorithms is part of future work. 
	
%	Whereas there is no restriction on entry/exit of the SUs in TSN and TDN algorithms and the SUs can enter or exit any time throughout the horizon as the newly entered SUs learn the channel characteristics in next $T_{CC}$ time slots after its entry based upon its channel selection and vacancy observations. Thus reduces the regret incurred during the $T_o$ duration of each epoch in MC algorithm.
%	
%	\item Collision: To estimate the number of SUs in the network, MC algorithm allows forced collision using randomly selection of the channels in the learning phase of each epoch resulting in significant loss of throughput and wastage of transmission power as each collision results in reprocessing and retransmission of the same (lost) packet. Whereas there is negligible number of collisions in our TSN and TDN algorithms due to sequential hoping used in the CC phase. 

	
\end{itemize}
